PR2: A Physics- and Photo-realistic Humanoid Testbed with Pilot Study in Competition

This paper presents the development of a Physics-realistic and Photo-realistic humanoid robot testbed, PR2, to facilitate collaborative research between Embodied Artificial Intelligence (Embodied AI) and robotics. PR2 offers high-quality scene rendering and robot dynamic simulation, enabling (i) the creation of diverse scenes using various digital assets, (ii) the integration of advanced perception or foundation models, and (iii) the implementation of planning and control algorithms for dynamic humanoid robot behaviors based on environmental feedback. The beta version of PR2 has been deployed for the simulation track of a nationwide full-size humanoid robot competition for college students, attracting 137 teams and over 400 participants within four months. This competition covered traditional tasks in bipedal walking, as well as novel challenges in loco-manipulation and language-instruction-based object search, marking a first for public college robotics competitions. A retrospective analysis of the competition suggests that future events should emphasize the integration of locomotion with manipulation and perception. By making the PR2 testbed publicly available at https://github.com/pr2-humanoid/PR2-Platform, we aim to further advance education and training in humanoid robotics. Video demonstration: https://pr2-humanoid.github.io/

==> jfr_config.tex <==
%\usepackage{amsmath,amssymb,mathabx}
\usepackage{mathtools}
\usepackage{lmodern}
\usepackage{tabularx}
%\usepackage{algorithmic}
% \usepackage{algpseudocode}
%\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{acronym}
\usepackage{enumitem}
\usepackage{booktabs}
\usepackage{hyperref}
\usepackage{bm}

% % \usepackage[stable]{footmisc}
% \usepackage{balance}
% \usepackage{xspace,setspace}
\usepackage{subcaption}
%\usepackage[skip=3pt,font=small]{caption}
\usepackage[capitalise]{cleveref}
\usepackage{tabularx,colortbl,multirow,array,makecell}
\usepackage{overpic}
%\usepackage{cite}
\usepackage{tikz}
\usepackage[]{mdframed}
\usepackage{xcolor,verbatimbox}
\usepackage{float}
% \let\labelindent\relax
%\input{configs}
% \makeatletter
% \DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
% \def\pmb{e.g.}{\emph{e.g}\onedot} \def\pmb{e.g.}{\emph{E.g}\onedot}
% \def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
% \def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
% \def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
% \def\wrt{w.r.t\onedot~} \def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot~}
% \def\pmb{PR2}{PR2~}
% \makeatother

%\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
%\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
%\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
%\crefname{figure}{Fig.}{Fig.}
\Crefname{figure}{Figure}{Figure}

\acrodef{rl}[RL]{Reinforcement Learning}
\acrodef{il}[IL]{Imitation Learning}
\acrodef{dof}[DoF]{Degree of Freedom}
\acrodef{ik}[IK]{Inverse Kinematics}
\acrodef{mpc}[MPC]{model predictive control}
\acrodef{wbc}[WBC]{whole-body control}
\acrodef{ros}[ROS]{Robot Operating System}
\acrodef{slam}[SLAM]{Simultaneous Localization and Mapping}
\acrodef{com}[CoM]{center of mass}
\acrodef{cam}[CAM]{centroidal angular momentum}
\acrodef{cmm}[CMM]{centroidal momentum matrix} 
\acrodef{cdm}[CDM]{centroidal dynamics model}
\acrodef{cop}[CoP]{Center of Pressure}
\acrodef{usd}[USD]{Universal Scene Description}
\acrodef{eai}[Embodied AI]{Embodied Artificial Intelligence}

\newcolumntype{x}{>{\columncolor{gblue}}l}
\newcolumntype{y}{>{\columncolor{gred}}l}
\newcolumntype{z}{>{\columncolor{LightOliveGreen}}l}

\definecolor{locomotion}{RGB}{179, 183, 238}  
\definecolor{manipulation}{RGB}{234, 154, 178} 
\definecolor{perception}{RGB}{235, 217, 252}  

\usetikzlibrary{tikzmark, calc}
% Makes a style for double color filling
\tikzset{
    double color fill/.code 2 args={
        \pgfdeclareverticalshading[%
            tikz@axis@top,tikz@axis@middle,tikz@axis@bottom%
        ]{diagonalfill}{100bp}{%
            color(0bp)=(tikz@axis@bottom);
            color(50bp)=(tikz@axis@bottom);
            color(50bp)=(tikz@axis@middle);
            color(50bp)=(tikz@axis@top);
            color(100bp)=(tikz@axis@top)
        }
        \tikzset{shade, left color=#1, right color=#2, shading=diagonalfill}
    }
}
% Code adapted from Gonzalo: https://tex.stackexchange.com/a/67096/81905
\newcommand\BGcell[4][0pt]{%
  \begin{tikzpicture}[overlay,remember picture]%
    \path[#4] ( $ (pic cs:#2) + (-.5\tabcolsep,1.9ex) $ ) rectangle ( $ (pic cs:#3) + (\tabcolsep,-#1*\baselineskip-.8ex) $ );
  \end{tikzpicture}%
}%
\newcounter{BGnum}
\setcounter{BGnum}{1}
\newcommand\cellBG[3]{
    \multicolumn{1}{
        !{\BGcell{startBG\arabic{BGnum}}{endBG\arabic{BGnum}}{%
                #1}
            \tikzmark{startBG\arabic{BGnum}}}
            #2
        !{\tikzmark{endBG\arabic{BGnum}}}}
        {#3} 
      \addtocounter{BGnum}{1}
}
% end of code from Gonzalo

\tikzset{%
    diagonal fill/.style 2 args={%
        double color fill={#1}{#2},
        shading angle=45,
        opacity=0.8},
    other filling/.style={%
        shade,
        shading=myshade,
        shading angle=0,
        opacity=0.5}
   }
